Heterogeneous federated collaborative filtering using FAIR: Federated Averaging in Random Subspaces

Recommendation systems (RS) for items (e.g., movies, books) and ads are widely used to tailor content to users on various internet platforms. Traditionally, recommendation models are trained on a central server. However, due to rising concerns for data privacy and regulations like the GDPR, federated learning is an increasingly popular paradigm in which data never leaves the client device. Applying federated learning to recommendation models is non-trivial due to large embedding tables, which often exceed the memory constraints of most user devices. To include data from all devices in federated learning, we must enable collective training of embedding tables on devices with heterogeneous memory capacities. Current solutions to heterogeneous federated learning can only accommodate a small range of capacities and thus limit the number of devices that can participate in training. We present Federated Averaging in Random subspaces (FAIR), which allows arbitrary compression of embedding tables based on device capacity and ensures the participation of all devices in training. FAIR uses what we call consistent and collapsible subspaces defined by hashing-based random projections to jointly train large embedding tables while using varying amounts of compression on user devices. We evaluate FAIR on Neural Collaborative Filtering tasks with multiple datasets and verify that FAIR can gather and share information from a wide range of devices with varying capacities, allowing for seamless collaboration. We prove the convergence of FAIR in the homogeneous setting with non-i.i.d data distribution. Our code is open source at {https://github.com/apd10/FLCF}

==> algorithms/algo1.tex <==
\begin{algorithm}[t]
\caption{\fair{}: Heterogeneous 
 Federated Averaging in Random Subspaces (SERVER) }\label{alg:algo1}
\begin{algorithmic}
\Require $N$ devices with data $\{\mathcal{D}_i\}_{i=1}^N$, capacity ratios $\{\alpha_i\}_{i=1}^N$, $0 < \alpha_i \leq 1$. Loss function $F(\theta, \mathcal{D})$. $\theta$ initial parameter vector at the server.
\vspace{5pt}
\State initialize $\theta$
\For {round t in (0,\dots,T) }  
    \State $\theta' \gets 0$ 
    \State \Comment{For updated value of theta after the round}
    \State Generate seed for hash function $h$
    \State $C \gets $ random set of clients
    \State Communicate seed to clients in C
    \State $\forall i \in C, S_i \gets $ projection matrix corresponding to capacity $\alpha_i$ according to equation \ref{eq:matrixcut}.
    \State \Comment{These matrices are not realized. Hashing is on the fly}
    \State $\psi_i \gets $ projection($S_i, \theta$) according   $\ref{eq:reduction}$ equation.
    \For{ each client $i$ in C in parallel}
    \State Send $\psi_i$
    \State $\psi_i' \gets $ wait for client update
    \State $\theta_i' \gets S_i \psi$ projection according to equation \ref{eq:recovery}
    \State $\theta' \gets \theta' + p_i \theta_i'$
    \State \Comment{ $p_i$ are the weights for weighted aggregation used in fed-avg, aggregation is atomic to avoid data race}
    \EndFor
    \State $\theta \gets \theta'$
\EndFor
\end{algorithmic}
\end{algorithm}




==> algorithms/algo2.tex <==
\begin{algorithm}[t]
\caption{\fair{}: Heterogenous 
 Federated Averaging in Random Subspaces (CLIENT $i$) }\label{alg:algo2}
\begin{algorithmic}
\Require Data $\mathcal{D}_i$, capacity $\alpha_i$ $0 < \alpha_i \leq 1$. Loss function $F_i(\theta, \mathcal{D})$. 

\State \textbf{Client Code (i):}
\State Receive seed for hash function $h$
\State Receive $\psi_i$
\State Optimize $F_i(\mathcal{D}_i, \psi_i) = F(\mathcal{D}_i, S_i\psi_i$ for $E$ epochs on local data $\mathcal{D}_i$ 
\State \Comment{ Training done in a memory-efficient manner using kernels from \cite{robe1}, \cite{desai2022efficient}  which use \ref{eq:partial} equation }
\State Send Updated $\psi_i$ to server.
\end{algorithmic}
\end{algorithm}


==> figures/datastats.tex <==
\begin{figure}
    \centering
    \begin{subfigure}{0.48\linewidth}
    \includegraphics[scale=0.27]{images/data_top_100user.png}
    \caption{Goodreads-S}
    \label{fig:my_label}
    \end{subfigure}
    \begin{subfigure}{0.48\linewidth}
    \includegraphics[scale=0.27]{images/data_top_100books.png}
    \caption{Goodreads-S}
    \label{fig:my_label}
    \end{subfigure}
    \begin{subfigure}{0.48\linewidth}
    \includegraphics[scale=0.27]{images/data_top_1000user.png}
    \caption{Goodreads-L}
    \label{fig:my_label}
    \end{subfigure}
    \begin{subfigure}{0.48\linewidth}
    \includegraphics[scale=0.27]{images/data_top_1000books.png}
    \caption{Goodreads-L}
    \end{subfigure}
    \caption{Data statistics. It can be seen that each user has lot of samples. There is a strong power-law in the number of samples available for each book.}
    \label{fig:datastats}
\end{figure}

==> figures/fedrz.tex <==
\begin{figure*}
    \centering
    \includegraphics[scale=0.2]{images/fedrz.png}
    \caption{(Left) Heterogeneous federated learning setup where full model parameters are stored on a server; however, fewer parameters can be stored on individual devices, and these capacities vary across devices. (Right) Illustration of operations in \name for the three steps. Every device, according to its capacity, has a parameter-sharing mapping function that defines a subspace inside which it searches for the solution. \textbf{Model download:} the entire server parameter vector (in $R^n$) is projected onto the device-specific subspace (of dimension $R^m$, $m < n$) (the operation can be performed on device/server), the basis of the projected parameter vector is changed, and the resulting $m$ dimensional vector is communicated. \textbf{Model training:} The parameter vector in the original basis can be recovered from the communicated parameters and used to train the model. Care is taken only to recover parts of the original parameter vector so that the entire parameter vector is never realized in memory. \textbf{Model upload:} The $m$ parameter transformed vector is communicated back to the server. The server changes the basis to the original basis and obtains the parameter vector in $R^n$. All such vectors obtained from different devices can be aggregated to obtain an updated server parameter vector.}
    \label{fig:my_label}
\end{figure*}

==> figures/paramsharing.tex <==
\begin{figure}
    \centering
    \includegraphics[scale=0.3]{images/paramsharing.png}
    \caption{The parameter sharing method of compression. The parameter-vector uses a small repository of weights in a shared manner.}
    \label{fig:my_label}
\end{figure}

==> sections.mod/abstract.mod.tex <==
Recommendation systems (RS) for items (e.g., movies, books) and ads are widely used to tailor content to users on various internet platforms. Traditionally, recommendation models are trained on a central server. However, due to rising concerns for data privacy and regulations like the GDPR, federated learning is an increasingly popular paradigm in which data never leaves the client device. Applying federated learning to recommendation models is non-trivial due to large embedding tables, which often exceed the memory constraints of most user devices. To include data from all devices in federated learning, we must enable collective training of embedding tables on devices with heterogeneous memory capacities. Current solutions to heterogeneous federated learning can only accommodate a small range of capacities and thus limit the number of devices that can participate in training. We present Federated Averaging in Random subspaces (\fair), which allows arbitrary compression of embedding tables based on device capacity and ensures the participation of all devices in training. {\fair} uses what we call \textit{consistent} and \textit{collapsible} subspaces defined by hashing-based random projections to jointly train large embedding tables while using varying amounts of compression on user devices. We evaluate {\fair} on Neural Collaborative Filtering tasks with multiple datasets and verify that {\fair} can gather and share information from a wide range of devices with varying capacities, allowing for seamless collaboration. We prove the convergence of {\fair} in the homogeneous setting with non-i.i.d data distribution. Our code is open source at {https://anonymous.4open.science/r/FAIR\_FederatedCollaborativeFiltering}.

==> sections.mod/abstract.tex <==
Recommendation models such as those for items (e.g., movies, books) and ads are crucial in enabling effective user interaction with the WWW. Traditionally, recommendation models are trained on a centralized server. However, due to rising concerns for data privacy and regulations such as the GDPR, federated learning is an increasingly sought paradigm to train machine learning models in a distributed fashion, with data always remaining on user devices. One key challenge in training and deploying most recommendation models on user devices is the storage of large embedding tables, such as for items or categorical data. The memory capacity of user devices often varies from device to device, and thus we must enable collective training of embedding tables on devices with heterogeneous memory capacities. Current solutions to heterogeneous federated learning can only accommodate a small range of capacities unsuitable for embedding tables in RS models. We present \longname (\fair), which allows arbitrary compression of embedding tables and ensures the participation of all devices in training. In this paper, we choose arguably the simplest setting of neural collaborative filtering and show that \fair{} is an excellent approach to training large embedding tables while using varying amounts of compression on user devices. We find that \fair{} provides an effective way to collaborate information from both low and high-capacity devices. We also show that while \fair{} is best suited for embedding tables, its recipe is general and can be extended to all model components. Additionally, we prove the convergence of \fair{} in the homogeneous setting with non-i.i.d data distribution. Our code is open source\footnote{https://anonymous.4open.science/r/FAIR\_FederatedCollaborativeFiltering}.

==> sections.mod/experiments.tex <==
\section{Experimental evaluation of FAIR}
% We ask the following research questions about FAIR. 
\begin{itemize}[leftmargin=*, nosep]
     \item \textbf{RQ1:}  Although existing heterogeneous federated learning solutions cannot cater to devices needing more compression, how does FAIR perform when compared to existing  baselines in lower compression regime? 
     \item \textbf{RQ2:} Can FAIR cater to situations where existing baselines cannot be applied? Can FAIR include devices that require sub-bit compression? (i.e more than 32$\times$ reduction of embedding table size)
    \item \textbf{RQ3:} Value of FAIR over ignoring data from devices that cannot fit the entire model.
    \item \textbf{RQ4:} Value of heterogeneous FAIR (FAIR-HET) (incorporating different sized models from devices) over homogenous FAIR (FAIR-HOM) which deploys the smallest model on all devices to incorporate all the data.
    \item \textbf{RQ5:} 
    
%     \item \textbf{RQ4:} How does FAIR perform when applied to general model components?
%     \item \textbf{RQ5:} How does FAIR perform with both explicit and implicit feedback based CF training?
\end{itemize}
The experimental setup is described below:

\textbf{Datasets:} We select standard recommendation datasets from the collection of datasets\footnote{https://cseweb.ucsd.edu/~jmcauley/datasets.html}. We choose the datasets with large number of items as our proposed method is for collaborative learning of heterogenous representation of these embedding tables across clients. Specifically, we choose Goodreads\cite{wan2018item}, AmazonProduct \cite{mcauley2015image, he2016ups}. In order to create feasible datasets for federated learning, we choose top $100$ users with most interactions and create a truncated version of dataset (these are denoted as Goodreads-100 and Amazon-100 datasets)

\textbf{Model:} We use the neural matrix factorization model NeuMF \cite{he2017neural} in our experiments. This model has two components: a generalized matrix factorization (GMF) module and a MLP module which are combined to make a score prediction. It maintains two embedding tables for users and items---one for each module. In our federated setup, each client model maintains its user embedding and copies of a suitably compressed item embedding table. We use number of factors equal to $8$.

\textbf{Task and metrics:} We evaluate FAIR on two tasks: implicit feedback based ranking and rating prediction for explicit feedback. \textbf{Implicit feedback:} We use the interaction datasets as implicit feedback, i.e. any interaction by user with an item is a positive instance and those items not interacted with are negative instances. We use Bayesian Personalized Ranking loss (BPR) \cite{rendle2012bpr} for training. We split the positive data into train and test sets. The model is trained with the train-split of positive data along with randomly sub-sampled negative instances from the set of all items (note that for training even items in test-split are negative). For evaluation, we rank all the items except train-split positive items and compute the \textit{normalized discounted cumulative gain} (ndcg@20) where gain of test-split positive item is $1$ and those of negative items is $0$. \textbf{Explicit feedback:} We train a NeuMF-MLP model for the rating prediction task with MSE as the metric.

\input{tables/implicit_table_1}
\input{tables/exp1-mod}
\input{tables/general-mod}

\textbf{Hyperparameter search:}
We search for the hyperparameters from the following choices: learning rate $(1e{-}1, 1e{-}2, 1e{-}3, 1e{-}4, 1e{-}5)$, batch size ($256, 512, 1024$), regularization weight for BPR loss ($1e{-}2, 1e{-}4, 1e{-}6$), dropout for MLPs ($0, 0.1, 0.25, 0.5$), number of local epochs in federated learning E($1, 2$). Hyperparameters are chosen by running federated setup for $50$  rounds and central setup for $20$ epochs.

\textbf{Baselines:} We consider the existing works on heterogenous capacity devices in federated learning, FEDHM\cite{yao2021fedhm} and HETEROFL \cite{diao2020heterofl} as baselines. We note that in context of embedding tables, FEDHM and HETEROFL are equivalent in terms of computation. This is discussed in more detail in appendix \ref{appendix:baselines}. Also, as FEDHM is recent and improves over HETEROFL , we use FEDHM as a baseline in our experiments. We also define more baselines. \apd{(1) FAIR-HOM : FAIR, TRUNC-DATA }

\textbf{Resources:} All experiments are performed on Quatro-RTX 8000 GPUs.

\textbf{Comparison with existing baselines and sub-bit compression (RQ1, RQ2)}:
From the table \ref{tab:implicit_table_1}, we can see that when collaborating with smaller capacity devices where we can deploy baselines, FAIR is competitive /  better  than baselines of FEDHM. Additionally, FAIR can collaborate with extremely small capacity devices where methods such as FEDHM or HETEROFL cannot be applied.  Additionally, FAIR can also incorporate devices that require sub-bit compression (i.e. more than 32$\times$ compression)


\textbf{Study of losing data due to heterogenous memory capacities (RQ3) }:
Discarding data from devices that cannot host the complete model can be catastrophic in cases of CF models as most devices do not have the ability to store entire embedding tables. We analyse the gains with FAIR over data-loss in table \ref{tab:data-loss}
\input{tables/data_loss}


\textbf{}







==> sections/abstract.tex <==
Due to rising concerns for data privacy, federated learning is an increasingly sought paradigm to train machine learning models in a distributed fashion, with data always locally situated on user devices. One of the interesting challenges faced by federated learning is learning models in a heterogeneous scenario where the computation, communication, and memory of the devices vary. Current solutions to heterogeneous federated learning can only accommodate a small range of capacities due to the inherent limitations of the approach. These methods fail, especially for recommendation models with huge embedding tables. We present a generic approach, called \longname (\namens), to deal with the heterogeneous memory capacity of devices in a principled manner allowing arbitrary compression of embedding tables. This is a first-of-its-kind study of learning embedding tables in a federated learning setting, let alone a heterogeneous setting. We propose a federated-embedding learning dataset derived from the publicly available Goodreads dataset. We show that \name is an excellent approach to obtaining compressed embeddings in a federated setting and also provides an effective way to collaborate information from both low and high-capacity devices. Additionally, we prove the convergence of \name in the homogenous setting with non-i.i.d data distribution.


==> sections/background.tex <==
\subsection{Federated learning}
% describe
Federated learning \cite{mcmahan2017communication} is a distributed training paradigm designed to preserve the privacy of the data on local user devices. In this paradigm, training occurs on the user devices. A server co-ordinates the training process: it sends model parameters to devices, devices train the model parameters on local data and upload updated parameters to the server which are then aggregated. The process is repeated for multiple rounds. In typical distributed training, the gradients from all devices are aggregated after each step. Communicating the gradients at each step is not feasible over wireless networks. Thus, in federated learning, each device trains for multiple steps (typically one or more epochs of local data) and communication happens in a staggered manner. Many algorithms have been proposed for aggregating these gradient updates, the most popular being FEDAVG \cite{mcmahan2017communication}, FEDProx \cite{li2020federated} where the model weights from each device are averaged to give updated model weights for the server.  

%heterogenous
There are many challenges in federated learning \cite{kairouz2021advances} which distinguishes it from traditional machine learning. One of the important challenges is handling heterogeneity in various forms. The different users might generate data with different distributions which breaks the standard i.i.d assumption of machine learning. Each device might have different storage and energy capacities, computation power, and communication bandwidths. The availability of each device for training might also vary from user to user which means we cannot randomly sample a user for training. In this paper, we deal with storage capacity and communication bandwidth heterogeneity which are the key bottlenecks for training embedding tables in a federated setting.




\subsection{Universal hash functions}
A hash function, usually denoted as $h:\mathbf{N} \rightarrow \{0,...,m-1\}$
for some $m \in \mathbf{N}$ is a function that maps a given integer into a range $m$. If a hash function is drawn from all possible functions, i.e. from a family of random hash functions, 
the hash values for any $k$ integers is independent. However, such a hash function would require storing the hash value for every input. Alternatively, there are restricted hash function families known as universal hash families \cite{carter1977universal} that require only $O(1)$ storage cost and $O(1)$ computation cost. However, this comes at a cost of reduced independence properties; the only guarantee these families provide is: 
\begin{equation}
    \mathbb{P}(h(a) == h(b)) \leq \frac{1}{m}
\end{equation}
This independence is practically enough in most cases \cite{mitzenmacher2008simple}. An instance of a universal hash family commonly used in practice is the following:
\begin{equation}
    h(x) = (Ax + B) \% P \% m
\end{equation}
where $P > m$ is a large prime. $A$ and $B$ are integers which are drawn randomly from $\{1,...,P{-}1\}$  and $\{0, ..., P{-}1\}$ respectively. It is clear from this example that the storage and computation cost for this function is $O(1)$.


\subsection{Random parameter sharing as a compression technique}
\input{figures/paramsharing.tex}
Random parameter sharing \cite{hashnet,robe1} is a popular compression technique, especially for embedding tables in recommendation models. Given a model with a parameter-vector $\theta \in R^n$, the idea behind this compression is to use a smaller repository of weights $\psi \in R^m$ and use only these weights repeatedly to form the complete parameter-vector $\theta$. The exact mapping from the indices of $\theta$ to indices of $\psi$ is usually a random hash function. Thus, in arguably the simplest form, using a hash function $h:\{0,..,n-1\} \rightarrow \{0,..m-1\}$:
\begin{equation}
    \theta[i] = \psi[h(i)] \forall i \in \{0,..,n-1\}
\end{equation}
More generally, one can recover $\theta$ using a linear projection matrix $\mathcal{S}$ as follows:
\begin{equation}
    \theta = \mathcal{S} \psi
\end{equation}

Efficient versions of parameter sharing were recently proposed in \cite{robe1}.

==> sections/convergence.tex <==
\input{figures/subspaces}
Recently, \cite{li2019convergence} proved $O(\frac{1}{T})$ convergence of federated learning on non-iid data with full and partial participation of devices when the following conditions (paraphrased from \cite{li2019convergence}) are met:
\begin{itemize}[nosep, leftmargin=*]
    \item \textbf{Assumption 1:} $F_1$, ... $F_N$ are L-smooth
    \item \textbf{Assumption 2:} $F_1$, .... $F_N$ are $\mu$-strongly convex
    \item \textbf{Assumption 3:} Variance of stochastic gradients on all the devices is bounded. If $\zeta_t^k$ is the stochastic sample for device $k$ at round $t$, then  $\mathbb{E} || \nabla F_K(\theta^k_t, \zeta_T^k) - \nabla F_K(\theta^k_t, \mathcal{D}_k) ||^2 \leq \sigma_k^2$
    \item \textbf{Assumption 4:} Expected squared norm of the stochastic gradients is uniformly bounded, $\mathbb{E}(|| \nabla F_k(\theta^k_t, \zeta^k_t ||^2 \leq G^2)$ for all devices and rounds
\end{itemize}
For the exact expression of convergence, we refer the reader to \cite{li2019convergence}. 

The convergence of \name under homogeneous conditions with full participation (alt. partial participation) can be stated as the corollary of the Theorem 1 ( alt. Theorem 2, 3). We first need two lemmas to complete the proof.

\begin{lemma}\label{lemma:assumption}
Under \name, using notations defined in Notation~\ref{not:name}, if $F_1, F_2..., F_N$ satisfy the above assumptions 1-4, and $F'_1, F'_2, ... F'_N$ where:
\begin{equation}
    F'_i(\psi) = F_i(\mathcal{S}\psi)  \qquad \forall i \in \{1,..,N\}
\end{equation}
And $\mathcal{S}$ is a orthonormal matrix, then $F'_1, F'_2, ... F'_N$ also satisfy the assumptions 1-4 with the same constants $L, \mu, \sigma_k, G$ for all $k\in \{1,...,N\}$.
\end{lemma}
Proof of Lemma \ref{lemma:assumption} is provided in the appendix. 

\begin{lemma}\label{lemma:server}
Under \name, using notations defined in Notation~\ref{not:name} and a unique sub-space matrix $\mathcal{S}$ across all the devices, the server parameter-vector $\theta_S$ can always be represented as: 
\begin{equation}
    \theta_S = \mathcal{S} \psi
\end{equation}
For some $\psi$. And the parameter aggregation equation can be written as follows,
\begin{equation}
    \psi = \sum_{i=1}^N  p_i \psi_i
\end{equation}
where $p_i$ are weights of aggregation as per standard FEDAVG.
\end{lemma}

With Lemmas~\ref{lemma:assumption} and \ref{lemma:server}, we can cast the entire federated learning with \name under homogeneous settings as federated learning with parameters in the subspace $\mathcal{S}$ (even at the server). Thus, the convergence of \name can be stated as a corollaries to Theorem 1,2,3 from \cite{li2019convergence}. We only state the concise form of Theorem 1 here:

\begin{corollary}
If the functions $F_1, ... F_N$ satisfy assumptions 1-4, then under homogeneous setting of \name (equal dimension of random subspace),  the algorithm converges at a rate $O(\frac{1}{T})$.
\end{corollary}




==> sections/dataset.tex <==
In this section, we propose a dataset to be used for evaluating embedding learning in a federated setting.

\input{tables/goodreads}
\input{figures/datastats.tex}
There are two main approaches to building embeddings in recommendation systems. In the first approach, embeddings of various items are created using information available for these items. Content includes natural language descriptions, images associated with the items, and media content. Generally, pre-trained models are used to encode the content. Another widely popular approach is that of large embedding tables \cite{dlrm}, where embeddings are learned from scratch using the interaction data between users and items in an end-to-end fashion. In practical applications, these embedding tables are enormous due to a large number of items. However, datasets that can capture this scale are few, if not none. Also, those datasets do not have user information that can be used to construct a natural federated dataset. Datasets such as MIND \cite{wu2020mind}, Adressa \cite{gulla2017adressa}, Movielens\footnote{https://grouplens.org/datasets/movielens/25m} and similar datasets are used in recent literature on federated recommendation \cite{yi2021efficient, luo2022personalized, wang2021fast, anelli2021federated}. However, these datasets are primarily used in a content-driven fashion or have a minimal number of items (see Table~\ref{tab:existing} in appendix).  Thus, in this section, we propose to use the dataset of ``Goodreads''\cite{DBLP:conf/acl/WanMNM19,DBLP:conf/recsys/WanM18}, which gives reasonably sized embedding tables for items and a good number of users for a naturally established federated setting.

\input{tables/baseline.tex}
\input{tables/exp1.tex}
\input{tables/inconsistent}
%\input{figures/subspaces.tex}
\textbf{Dataset generation:} We use the shelves portion of Goodreads dataset to generate our dataset. This file has the user interaction data with five fields ``user\_id,\hspace{4pt}book\_id,\hspace{4pt}is\_read,\hspace{4pt}is\_review,\hspace{4pt}rating". We only use this data for rating prediction. In order to generate smaller datasets with restricted number of users, we choose the users with most interactions. ``Goodreads-S" is generated using the top 100 users and ``Goodreads-L" using the top 1000 users. The data statistics per user and per book in these datasets is shown in \ref{fig:datastats}. It should be noted that most users have very little data as is typical in large embedding table training. 



\textbf{Model and FedAVG settings and results:}
We propose to use a recommendation model that captures the core problem of embedding table learning. We use the two-tower model. In this model, the server contains a user embedding table, a book embedding table, and optional embedding tables for is\_read and is\_review. All of the embeddings are concatenated and passed through a MLP 10-10-1. The model is trained for rating prediction as a regression problem. We use the number of epochs at every round (E) to be 1 (higher values do not perform well), a sample size of devices ($K$) to be 10, and run the federated regression for 1000 rounds. We present results with different embedding table sizes in Table \ref{tab:baseline}.






==> sections/experiments.tex <==
%In this section, we perform various studies to evaluate \name in different settings. 
%We also perform ablation studies to assess our findings and choices. 

% \textbf{Server MSE with \namens:}
% The server MSE for different homogeneous and heterogeneous settings is shown in Table \ref{tab:server-fair}. We make the following observations:
% \input{tables/general.tex}

% \begin{itemize}[nosep, leftmargin=*]
%     \item Under homogeneous settings, the compression given by \name is better than the compression obtained by naive slimming of the embedding table. For example, an embedding table of dimension 32 compressed by $4\times$ (i.e., an effective dimension of 8) gives a MSE of 0.6701, while an embedding table of dimension 8 gives a MSE of 0.7277. This is consistent for higher compression ratios as well.
%     \item The server MSE for heterogeneous settings of the form ``$M_1\times$-$M_2\times$" (M1 $<$ M2) compressions are better than using only ``$M_2\times$". This is consistent across different compression regimes. One would expect this to happen as richer information is received from devices with $M_1\times$. Surprisingly, the server accuracy for ``$M_1\times$-$M_2\times$" is even better than using ``$M_1\times$" across the board. For example, in ``$16\times$-$32\times$", the server model gives a MSE of 0.6716, which is better than both the ``$16\times$" (0.6891) and the ``$32\times$" (0.6907) settings. We suspect this happens due to some form of regularization. Understanding this regularization of collaborative training in consistent and collapsing subspaces is left for future work.
%     \item The convergence with \name for the server is faster for higher compression ratios in both homogeneous and heterogeneous settings. We leave the theoretical analysis of the effect of \name on convergence for future work.
%     \item LowRank methods are unsuitable for embedding tables as they cannot give compression ratios of ``$d\times$" and beyond, where $d$ is the embedding dimension and thus cannot cater to smaller capacity devices. In settings where LowRank can be implemented, \name outperforms LowRank in both homogeneous and heterogeneous settings.
% \end{itemize}
% \textbf{Local model quality with \namens:}
% In heterogeneous settings, one alternative procedure for devices with higher capacities is to restrict aggregation to only include updates from other devices with equal or higher capacities and ignore updates from devices with lower capacities. The rationale might be to keep things simple and algorithms like FEDAVG applicable or to avoid hurting the local model by adding noisy estimates from compressed models. However, as we find in Table \ref{tab:ablation}, with \namens, collaboration with lower-capacity devices leads to a better local model. The devices with ``$2\times$" compression give a better MSE when using updates from all devices across a range of compression ratios (ranging from $2\times$-$64\times$) than using only devices with a maximum compression of ``$2\times$" or ``$4\times$".
% \input{tables/ablation1.tex}

% \textbf{\name applied to general models:} The technique introduced in \name is general and can be extended to other models with different components, such as MLPs and Convolution. In this subsection, we show that \name is a practical approach for general models in heterogeneous and homogeneous settings. By using \namens, we reduce the communication and memory storage of modules like MLP and convolutions, but we do not change the underlying computation. The server accuracy for different homogeneous and heterogeneous settings are shown in Table \ref{tab:general}.

% Datasets and models: We perform experiments on two datasets: MNIST \cite{lecun1998mnist} and FEMNIST \cite{caldas2018leaf}. The MNIST data is generated using Non-i.i.d Dirichlet distribution \cite{caldas2018leaf} with 30 devices. We use E=20, T=200, K=10 for MNIST. FEMNIST, on the other hand, is a naturally partitioned extended MNIST data. Again we use E=20, T=200, and K=10. We use MLP 784-512-1 for MNIST and LeNet \cite{lecun2015lenet} for FEMNIST. We make the following observations:

% \begin{itemize}[nosep, leftmargin=*]
%     \item Under both homogeneous and heterogeneous settings and across all compression settings, \name achieves higher accuracy than LowRank on the FEMNIST dataset. 
%     %Additionally, in all but the highest compressions ratios, \name performs better than full FEDAVG. \apd{why?}
%     \item \name remains competitive with both LowRank and full FEDAVG on the MNIST dataset across a wide range of compression settings. For example, at all compression settings except ``$64\times$'', the server accuracies of \name and LowRank differ by $\leq 0.003$.
%     \item \name can employ compression ratios beyond the capability of LowRank and still achieve reasonable accuracy. For example, at a compression setting of ``$64\times$" \name reaches an accuracy of 0.7114 on the FEMNIST dataset compared with full FEDAVG achieving an accuracy of 0.7491. At the same time, LowRank cannot accommodate this compression level with the same model. 
    
%     \item For both MNIST and FEMNIST datasets, the server accuracy for heterogeneous settings of the form ``$M_1\times$-...-$M_n\times$" are better than homogeneous settings using only ``$M_n\times$." This behavior is expected as richer information is received in the updates from devices with greater capacities than $M_n\times$. 
%     %However, the opposite occurs in the FEMNIST dataset, where the server accuracy for heterogeneous settings of the same form performs worse than homogeneous settings using only ``$M_n\times$". We suspect that the regularization we hypothesized in Section 6.1 has a more significant effect on the model used in the FEMNIST experiments than the MNIST experiments. However, further exploration of the trade-off between relative information richness and regularization benefits in different compression schemes is left for future work. 
% \end{itemize}





% % In this section, we experimentally evaluate \namens. We perform a series of experiments to test various aspects of the proposal. 
% % \subsection{\name for embedding compression}

% % We will use Goodreads-S dataset\ref{sec:dataset} throughout the experimental section. We provide all the information in a single table \ref{tab:exp1} and conclude by comparing different settings. We run the following settings.
% % \begin{itemize}[nosep, leftmargin=*]
% %     \item \textbf{$\mathbf{\mathcal{C}_1}$-all:} All models are run with capacity $\mathcal{C}_1$. The server model is updated using FEDAVG on compressed models.
% %     \item \textbf{$\mathbf{\mathcal{C}_1{-}\mathcal{C}_2}$-\name:} First half of the devices use $\mathcal{C}_1$ and rest use $\mathcal{C}_2$ but they collaborate information via \namens. The server model is updated using FED-\name
% %     \item \textbf{$\mathbf{\mathcal{C}_1}$-only:}First half of the devices use $\mathcal{C}_1$ and do not collaborate with the rest devices (as they cannot accommodate $\mathcal{C}_1$ sized embedding table. The server model is updated only sing $\mathcal{C}_1$ devices.
% % \end{itemize}
% % The results of this experiment for different settings is shown in Table~\ref{tab:exp1}. We make the following observations.
% % \begin{itemize}[nosep, leftmargin=*]
% %     \item \textbf{Value of parameter sharing in homogeneous setting}. We can see that as we reduce the capacity of the models, the global server quality decreases at first, but then increases and even improves over baseline model. This happens due to two reasons. Firstly higher compression leads to better regularization which avoids early overfitting letting model to learn for longer times ( this can be seen in ``rounds" in table \ref{tab:exp1} ). Secondly, in large embedding tables, available training data per embedding is less. In such cases, parameter sharing improves learning of tail embeddings. 
% %     \item \textbf{Value of collaboration in heterogeneous setting}
% %     If we compare settings of the form $\mathcal{C}_1$-all, $\mathcal{C}_2$-all, $\mathcal{C}_1{-}\mathcal{C}_2$-\name where $\mathcal{C}_1 \geq \mathcal{C}_2$ We observe the following behavior consistently,
% %     \begin{itemize}
% %         \item  In terms of server model quality, $\mathcal{C}_1{-}\mathcal{C}_2$-\name outperforms $\mathcal{C}_1$ and $\mathcal{C}_2$ both consistently. This means that the better model ( bigger or smaller model might be better at different capacities ) influences the global server quality. In fact, the $\mathcal{C}_1{-}\mathcal{C}_2$-\name performs extra-ordinarily better. This might be an effect of \name on the optimization algorithm where we are communicating between parallel optimizations run in different subspaces.
% %         \item The local accuracy on first half of the devices (which can host $\mathcal{C}_1$ capacity ) is better when using $\mathcal{C}_1{-}\mathcal{C}_2$-\name than when we depoly $\mathcal{C}_1$-all , $\mathcal{C}_2-all$ and $\mathcal{C}_1$-only. Thus the local models get benefit potentially from regularization, optimization and data of the second half of devices. 
% %     \end{itemize}
% % \end{itemize}

==> sections/intro.tex <==
% federated learning for recommendations

Federated learning \cite{mcmahan2017communication} is a distributed model training paradigm devised for preserving data privacy. Recently, strict regulations on sharing user data with a centralized server have hampered machine learning models' quality, especially recommendation systems. Sub-standard recommendation models directly impact the user experience and efficiency on the various content-providing platforms. Thus, federated learning for recommendation models is the need of the hour. While many works such as  \cite{anelli2021federated,fedrec1,fedrec2,yi2021efficient} have talked about different aspects of federated learning, recommendation models with large embedding tables \cite{dlrm,guo2017deepfm} present a new challenge unexplored in literature. In arguably the most simple setting, a recommendation model consists of a user-embedding table and an item-embedding table. In a federated setting, a user-embedding table naturally distributes over user devices. Each user can train and store its embedding and does not need access to the other users' embeddings. However, for an effective system, it is essential to train item-embeddings collaboratively. The size of the item-embedding table makes it challenging to store and communicate these embedding tables during federated learning. Thus, federated learning for recommendation models needs innovative solutions. 

% heterogenous + existing solutions issues
Model heterogeneity is natural in recommendation models, where we want to build an embedding table of size $n \times d$ on the server. Still, the user devices can only store either a part or a compressed version of the embedding table. Additionally, different devices might have various capacities to store embedding tables. It is an interesting research question to see if we can collaborate effectively among heterogeneous devices. More importantly, among devices with varying capacities, how devices with low capacity can benefit devices with high capacity and vice-versa.

% existing solutions issues + our proposal
Recently, a few works have discussed federated learning in heterogeneous settings \cite{diao2020heterofl,hong2022efficient,yao2021fedhm}. Compression techniques such as low-rank decomposition \cite{yao2021fedhm}, sparse sub-network \cite{hong2022efficient}, and slimming models \cite{diao2020heterofl} form the key ideas behind these solutions. However, these solutions are not effective for large embedding tables. Specifically, these ideas can only give us embedding table representations that still require $O(n)$ capacity for a $n \times d$ embedding table on the server, and $O(n)$ is still too large in most cases. We propose the \longname(\namens) approach, which provides us with (1) an arbitrary control over embedding table sizes on devices with linear impact on communication costs and (2) the ability to effectively collaborate among devices with different-sized representations of embedding table. We leverage existing ideas in parameter sharing-based compression \cite{hashnet} in embedding tables to achieve the ability to perform federated learning of embedding tables under heterogeneous settings.

% Details of our method
Embedding compression in traditional machine learning using parameter-sharing techniques has gained a lot of traction due to the significant compression rates they can achieve \cite{robe1,robe2}. These techniques are part of a broader set of methods that can be applied to any generic model \cite{hashnet}. The parameter sharing techniques which reduce the original parameter space of $R^n$ to a reduced parameter space of $R^m$ can be interpreted as searching for the solution in a $m$-dimensional subspace inside $R^n$. By reducing the effective dimension of search and cleverly choosing a subspace, these methods reduce the memory requirement of the model. This paper is the first to extend these ideas to federated learning settings with homogeneous and heterogeneous scenarios. However, the naive application of existing parameter-sharing methods, where compressed models are stored on devices, does not perform well. In our approach \namens, we introduce the concept of consistent and collapsing subspaces to minimize the error during federated averaging of the models. Under \namens, we have two key ideas (1) \textbf{consistency:} every device with the same capacity shares the same random subspace in which it looks for solutions, and (2) \textbf{collapsing subspaces:} devices with different capacities have random subspaces that are contained in one another. We show that under these conditions in a  homogeneous setting, \name is guaranteed to converge at a rate $O\left(\frac{1}{T}\right)$ even with non-i.i.d data using a recent convergence result from \cite{li2019convergence}.

While the general focus of this paper is embedding tables, the technique we introduce is applicable to general models as well. We show that we achieve better results with \name in different homogeneous and heterogeneous settings than corresponding baselines such as federated low-rank methods \cite{yao2021fedhm} across the tasks of image classification and rating prediction. We also show that \name can handle extremely low capacities (higher compression ratios) on devices beyond the scope of existing solutions to heterogeneous federated learning.


==> sections/method.tex <==
\textbf{Notation}: We will use the following notation throughout the paper. The total number of devices is $K$, and in each round of federated learning, we will be sampling $k$ devices. We will denote devices by $D_1, ... D_K$. Let the server's parameters be represented by $\theta_S$ ($n=|\theta_S|$ ) and parameters stored at device $D_i$ be denoted by $\theta_i$ ($m_i=|\theta_i|$). Each device $D_i$'s capacity to store the embedding table is noted as the fraction of the total server parameters, $\mathcal{C}_i$, they can accommodate. For example, the number of parameters of the device $D_i$ is $|\theta_i| = \mathcal{C}_i |\theta_S| $. Let each device have two hash mapping function $\mathcal{H}_i : \{0,..,n-1\} \rightarrow \{0,..,m_i-1\}$ $\mathcal{G}_i : \{0,..,n-1\} \rightarrow \{\pm 1\}$. We use universal hash functions so that $\mathcal{H}_i$ can be stored in $O(1)$  memory. The $m_i$ dimensional subspace in $R^{n}$ defined by $\mathcal{H}_i$ be denoted by the column space of matrix $\mathcal{S}_i : n \times m$, where  $\mathcal{S}_{i}[a,b] = \mathcal{G}_i(a) \textrm{ iff } \mathcal{H}(i) = j$. $\mathcal{S}_i$ defines the orthogonal basis of the subspace associated with parameters of device $\mathcal{D}_i$

\subsection{Parameter sharing as search in a subspace}
It would be useful for subsequent sections to understand the interpretation of parameter sharing as optimizing the model while looking for solutions in a subspace. Let the loss function be $\mathcal{F}(\theta_S)$ where $\theta_S \in R^n$ is the full set of parameters. (We re-use $\theta_S$ notation to be used for server parameters as they represent full parameters) In parameter sharing we use parameters from a smaller vector $\theta \in R^m$. We use the parameter sharing as described in \ref{sec:background} with hash functions $\mathcal{H}$ and $\mathcal{G}$, 
Let $\mathcal{S}[a,b] = \mathcal{G}(a)$ iff $\mathcal{H}$ and all other entries of $\mathcal{S}$ be zero. Then we can represent the relation between $\theta_S$ and $\theta$ using a random mapping matrix $\mathcal{S}$,
\begin{equation}
    \theta_S = \mathcal{S} \theta
\end{equation}

While optimizing the model $\mathcal{F}(\theta_S)$ under parameter sharing, we are essentially optimizing $\mathcal{F}(\mathcal{S} \theta)$. Thus, we are optimizing for a solution inside the column space of $\mathcal{S}$. Thus parameter sharing is essentially reducing the search space to $m$-dimensional subspace inside $n$-dimensional space and choosing a subspace that can be defined by hash functions and thus does not need explicit storage.

The columns of $\mathcal{S}$ provide an orthogonal basis for the column-space of $\mathcal{S}$. It is easy to see that every row of $\mathcal{S}$ has only one non-zero. Thus all the column-vectors are orthogonal to each other.

\subsection{\longname(\namens)}
There are three steps in federated learning (1) \textbf{download}: the server sends the model to the devices, (2) \textbf{train}: devices train their local models for some epochs, (3) \textbf{upload}: models send the updated parameters to the server, where all parameters are aggregated into a single model. We will explain how these three things happen in \name.

\paragraph{Phase 1: Download}
In this step, server sends its model parameters to sampled devices for this round. For device $\mathcal{D}_i$ parameters of the server $\theta_S$ are projected to the column-space of $\mathcal{S}_i$ and we use the columns of $\mathcal{S}_i$ to represent the $\theta_i$. The $\theta_i$ is then communicated to device $D_i$. The projection $\theta_i$ can be computed as follows,
\begin{equation}
    \theta_i[b] = \frac{\sum_{a, \mathcal{H}(a) {=} b} (G[a] \theta_S[a])}{ \sum_{a, \mathcal{H}(a) {=} b} 1}
\end{equation}
In order to change basis of the projected parameter vector to original space, we can simply use $\mathcal{S}_i \theta_i$.

\begin{theorem} (informal)
The computed vector $\mathcal{S}_i\theta_i$ is projection of $\theta_S$ on the column space of $\mathcal{S}_i$
\end{theorem}
The proof of above theorem is presented in appendix.
The computation of $\theta_i$ can either happen locally in case server broadcasts the model parameters to devices, or it can be performed on server and sent to devices. The server stores the hash functions $\mathcal{H}_i, \mathcal{G}_i$ for each device which takes $\mathcal{O}(1)$ space per hash function.

\paragraph{Phase 2: Training} The local training on each device $D_i$ proceeds using $\theta_i$. In principle, the model on the device is the same functional form as model on server using parameters $\mathcal{S} \theta_i$. However, the complete parameter vector in $R^n$ is never realized. Only partial recovery is made as is needed in every training step. For example, in case of embedding table, we only recover the embeddings for tokens present in the batch to be used inside the model. 


\paragraph{Phase 3: Upload and aggregation} The local weights $\theta_i$ are communicated to the server as is. At the server, using the hash functions $\mathcal{H}_i$ and $\mathcal{G}_i$ we can compute the parameters in original space using 

\begin{equation}
    \Tilde{\theta}_S^{(i)}  = \mathcal{S}_i \theta_i
\end{equation}

The final aggregated server weights are then computed as a weighted sum of all the model parameters received from the different devices as would be done in standard federated averaging.
\begin{equation}
    \theta_S  = \sum_{i\in {0,...k-1}} p_i \Tilde{\theta}_S^{(i)}
\end{equation}
where $p_i$ is the weight for device $i$ which is generally computed as ratio of number of samples in the data for this device to total number of samples across the devices involved in this round.

\subsection{Consistent and collapsing subspaces}
The previous subsections outlines the various operations involved in \name given the hash functions of each device. However, choosing the correct hash functions. \apd{As we will see in experiments and theory, the choice of hash functions is crucial of the federated averaging to converge}. Thus in \name we propose the following, 
\begin{itemize}
    \item consistency: if two devices share the same capacity, we use same hash functions $\mathcal{H}$ and $\mathcal{G}$ for them. (i.e both of the devices have the same solution subspace defined by $\mathcal{S}$)
    \item collapse: if any two devices have two different capacities $\mathcal{C}_1$ and $\mathcal{C}_2$ , $\mathcal{C}_1 < \mathcal{C}_2$, then we choose the hash functions $\mathcal{H}_1, \mathcal{G}_1, \mathcal{H}_2, \mathcal{G}_2$ such that $\mathcal{S}_1 \subset \mathcal{S}_2$.
\end{itemize}

We design our hash functions in a manner that above two properties are satisfied. Consider $K$ devices with capacities $\{ m_i\}_{i=1}^K$. We assume here that the capacities are powers of two. Let $m=\textrm{max}(\{ m_i\}_{i=1}^K)$. We define select random hash function $\mathbf{\mathbb{H}}: \{0,..,n-1\} \rightarrow \{0,..,m-1\}$ and $\mathbf{\mathbb{G}} : \{0,..,n-1\} \rightarrow \{\pm 1\}$. Then the hash functions for each device $D_i$ is defined as,
\begin{equation}
    \mathcal{H}_i(a) = \mathbb{H}(a) \% m_i \qquad \mathcal{G}_i = \mathbb{G}
\end{equation}
\begin{theorem}(infomal) 
The system of hash functions $\{\mathcal{H}_i\}_{i=1}^K$ and $\{\mathcal{G}_I\}_{i=1}^K$ define a consistent and collapsible system of subspaces.
\end{theorem}

\paragraph{Cost benefits associated with \name}
The \name method for heterogenous devices has two main benefits in terms of costs, 
\begin{itemize}[nosep, leftmargin=*]
\item The memory usage of each device is its parameter size $m_i = |\theta_i|$. So memory usage reduces by the factor of compression.
\item The communication cost of each device is proportional to its parameter size $m_i = |\theta_i|$, so the communication cost is reduced by the factor of compression. Also, note that this is true while applying \name to any generic model. 
\item The computation cost of each device is same (modulo the hashing cost which is minimal) as the original computation of full model. In context of embedding tables this is irrelevant as there is no computation involved in embedding tables and the main issue with embedding tables is the memory usage.
\item Hashing costs are additional costs that devices have to bear. In context of embedding tables, getting an embedding of dimension $d$ with chunk size $Z$, requires computing $d/Z$ hash computations,each of which are $O(1)$.
\end{itemize}

==> sections/method_1.tex <==

\paragraph{Notation (Federated learning):} We will use the following notation throughout the paper. The total number of devices is $N$, and in each round of federated learning, we will be sampling $K$ ($K \leq N$) devices. The  learning is run for $T$ rounds; each of which consists of $E$ steps of SGD. The optimization function associated with each device and its data is denoted as $F_i(\theta, \mathcal{D}_i)$ where $\theta$ is the parameter vector and $\mathcal{D}_i$ is the data associated with device $i$.

\paragraph{Notation (\namens):} \label{not:name}
Under \namens, we denote the server parameter-vector as $\theta_S \in R^n$. Each device $i$ has a capacity $0 < \alpha_i \leq 1$ and stores a parameter vector $\psi_i \in R^{m_i}$ where $ m_i= \alpha_i n$. Each device is associated with a subspace of dimension $m_i$, which is denoted by the column-space of an orthonormal (column) matrix $\mathcal{S}_i : n \times m_i$. The optimization functions of device $i$ are denoted as $F'_i(\psi_i, \mathcal{D}_i) = F_i(\mathcal{S}_i \psi_i, \mathcal{D}_i)$. Thus $\mathcal{S}_i$ is also the change-of-basis matrix. We denote $\theta_i = \mathcal{S}_i \psi_i$. $\theta_i$ and $\psi_i$ are same vectors in different basis. We call the basis of $\theta$ the server-basis and that of $\psi$ the device-basis.

We define the following property of the set of sub-spaces (equivalently orthonormal matrices): 

\begin{definition}[\textbf{Consistent \& Collapsible Sub-spaces}]
A given set of sub-spaces defined by columns of matrices $\{\mathcal{S}_i\}_{i=1}^N$  where $\mathcal{S}_i : n \times m_i$ matrix, is consistent if for every pair $i,j$, if $m_i = m_j$. then column-space of $\mathcal{S}_i$ is the same as the column-space of $\mathcal{S}_j$. Also, if $m_i < m_j$, then $\textrm{column-space}(\mathcal{S}_i) \subset \textrm{column-space}(\mathcal{S}_j)$.
\end{definition}

Next, we describe a single round in our proposed approach \namens.

\subsection{\longname}
There are three steps in federated learning for each round. A subset of $K$ devices is sampled from all devices. 
\begin{itemize}[nosep, leftmargin=*]
    \item \textbf{Model download}: The server sends the model to the sampled devices
    \item  \textbf{Local train}: Devices train their local models for some E iterations
    \item \textbf{Model upload and aggregate}: Models send their updated parameters to the server, where all parameters are aggregated into a single model
\end{itemize}

Each device is associated with a orthonormal matrix $S_i: n\times m_i$ where $m_i = \alpha n$ is the capacity of the device. The set of all these sub-spaces defined by matrices $\{S_i\}_{i=1}^N$ is chosen in a way that it is \textit{consistent and collapsible}. The basic steps of federated learning are present in \name along with additional strategy specific operations. We describe each of them below.
\input{figures/fedrz.tex}
\paragraph{Phase 1: Model download}

The server broadcasts the model parameter $\theta_S$ to the $K$ devices and each device $i$ 
 first projects $\theta_S$ onto its own subspace to get $\theta_i$ and changes the basis to obtain $m_i$ dimensional vector $\psi_i$. This can be performed directly by: 
 \begin{equation}
     \psi_i = \mathcal{S}_i^\top \theta_S  \label{eq:agg}
 \end{equation}
Alternatively, the server can perform this computation and only communicate $\psi$ to the device in a peer to peer network.

\paragraph{Phase 2: Local training} The local training on each device $D_i$ proceeds using $\psi_i$. The optimization function is $F'_i(\psi_i) = F_i(\theta_i)$. Thus, the functional form of the model on device is the same as that of the model on the server. One can think of the computation on the device as first recovering the $\theta_i$ in server-basis and then computing the function $F_i(\theta_i)$. However, the complete vector $\theta_i$ is never realized on the device. Only the partial vector is realized as needed during the computation of the function. For instance, 
in an embedding table, we only need access to some particular embeddings. In order to get embedding parameters located at, say $\theta_i[a:b]$, we can recover them using: 
\begin{equation}
    \theta_i[a:b] = \mathcal{S}[a:b,:] \psi_i
\end{equation}
Similar operations can be defined for parts of different model components such as matrices in MLP etc.

\paragraph{Phase 3: Upload and aggregation} In this step, the local weights $\psi_i$ in local-basis are communicated to the server. The sever changes the basis to server-basis and gets a potential updated server weight:
\begin{equation}
    \theta_i = \mathcal{S}_i \psi_i
\end{equation}

The final aggregated server weights are then computed as a weighted sum of all the model parameters received from the different devices as would be done in standard federated averaging:
\begin{equation}
    \theta_S  = \sum_{i\in {0,...k-1}} p_i \theta_i
\end{equation}
Where $p_i$ is the weight for device $i$ which is generally computed as ratio of number of samples in the data for this device to the total number of samples across all devices involved in this round.

\subsection{Consistent and collapsible sub-spaces with universal hash functions}
\input{figures/matrixfolding.tex}
In order to implement the above operations specific to \namens, it is important to make storage of $\mathcal{S}$ and computations involved with $\mathcal{S}$ cheap. In this section we show how to build consistent and collapsible sub-spaces using universal hash functions. Let $m = \max({m_i = \alpha n}_{i=1}^N)$. We draw two random hash functions $\mathcal{H}:\{ 0,...,n-1\} \rightarrow \{0,...m-1\}$ and $\mathcal{G}: \{0,...,n-1\} \rightarrow \{ \pm 1 \}$ from universal hash function families. We assume that $m_i$ are powers of two. If capacities are not power of two, then we can use the capacity to be highest power of two less than actual capacity. The set of sub-spaces is then defined as follows. Let each device have a sub-space represented by a orthogonal matrix $S_i$ (not orthonormal) We define $S_i: n \times m_i$ as follows:
\begin{equation}
    S_i[a,b] = \mathcal{G}(a)  \quad \textrm{iff} \quad \mathcal{H}(a) \% m_i {=} b   \label{eq:matrixcut}
\end{equation}

Note that each row of $S_i$ only has one non-zero element that is either $\pm 1$. Thus, each column of $S_i$ is orthogonal to every other column. We can convert this matrix into an orthonormal matrix by normalizing each column to 1.

\begin{theorem}
The set of sub-spaces $\{S_i\}_{i=1}^N$ of dimensions $\{m_i\}_{i=1}^N$ created using hash functions $\mathcal{H}$ and $\mathcal{G}$ as per equation \ref{eq:matrixcut}, is a consistent and collapsible set of sub-spaces.
\end{theorem}

The computation is illustrated in figure \ref{fig:marixfolding}. Essentially, we first create a matrix $S$ which is of dimensions $n \times m$. Then, in order to create the matrix $S_i$ for subspace $i$, we cut the matrix in columns of width $m/m_i$ and add the pieces together. This also provides an intuition for why this set of sub-spaces is collapsible: given any two matrices $S_i$ and $S_j$, if $m_i < m_j$, then each column of $S_i$ is sum of $m_j/m_i$ columns of $S_j$ and hence, column-space($S_i$) $\subset$ column-space($S_j$).

\paragraph{Cost considerations} With the choice of sub-spaces using universal hashing, the following are the costs associated with hashing at various steps:
\begin{itemize}[nosep, leftmargin=*]
    \item The matrices $\mathcal{S}$s do not need to be stored explicitly; they are implicitly defined and computed using hash functions $\mathcal{H}$ and $\mathcal{G}$. These hash functions can be stored in $O(1)$ memory. Thus, minimal storage cost is added to both the devices and server due to sub-space matrices. 
    \item Computation cost to project $\theta_S$ to column-space ($\mathcal{S}_i$) is $O(n)$.For each parameter of the vector $\theta_S$, we apply hash functions $\mathcal{H}$ and $\mathcal{G}$ to its index, say a, and add the value to the location $\mathcal{H}(a)$ multiplied by $\mathcal{G}(a)$. Each hash computation is $O(1)$ and thus, the overall computation is $O(n)$. This is also a cost included once per round, so it has little contribution in terms of amortized cost per training cycle.
    \item The cost of the server-side change-of-basis operation is also $O(n)$, with similar reasoning.
    \item The total cost of partial recovery of parameters in server-basis is proportional to the number of times a parameter is accessed in the implementation of the original function. For each access, we compute the the hashes $\mathcal{H}$ and $\mathcal{G}$. With efficient codes such as matrix multiplication, the number of operations performed per access is generally large and hence this cost is low w.r.t the total computational cost. The cost can be further reduced by using cache-efficient methods in parameter sharing. 
\end{itemize}


==> tables/ablation1.tex <==
\begin{table}
\centering

\caption{\textbf{Local MSE of devices with ``$2\times$" compression ratio:} This is an ablation study to measure the decrease in MSE for devices with $2\times$ compression when they incorporate updates from devices with greater compression. The two compression settings shown involve sorting the devices in order of decreasing data per device and subsequently partitioning the devices into six groups with an (almost) equal number of devices per group. The first compression setting ``$2\times$-$4\times$-..." assigns a $2\times$ compression ratio to the group with the most data per device, followed by a $4\times$ ratio to the group with the second most, and so on. The setting ``$64\times$-$32\times$-..." assigns a $64\times$ compression ratio to the group with the most data per device, followed by a $32\times$ ratio to the next group, and so on. \vspace{4pt}}
\label{tab:ablation}
\begin{tabular}{|cccc|}
\hline
\multicolumn{4}{|c|}{\textbf{FAIR Test MSE of Devices with 2x compressed tables}}                               \\ \hline
\multicolumn{1}{|c|}{}                     & \multicolumn{3}{c|}{\textbf{Max Collaboration COMP}}               \\ \hline
\multicolumn{1}{|c|}{\textbf{COMP}}        & \multicolumn{1}{c|}{Any}    & \multicolumn{1}{c|}{4x}     & 2x     \\ \hline
\multicolumn{1}{|c|}{2x-4x-8x-16x-32x-64x} & \multicolumn{1}{c|}{0.5649} & \multicolumn{1}{c|}{0.5697} & 0.6748 \\ \hline
\multicolumn{1}{|c|}{64x-32x-16x-8x-4x-2x} & \multicolumn{1}{c|}{0.8007} & \multicolumn{1}{c|}{0.8104} & 0.8118 \\ \hline
\end{tabular}
\end{table}

==> tables/existingdatasets.tex <==
\begin{table}[h]
\caption{Common datasets used in federated recommendation settings}
\centering
\label{tab:existing}
\begin{tabular}{|l|l|l|}
\hline
Dataset                           & \#users & \#items \\ \hline
MIND \citep{wu2020mind}          & 94K     & 65K     \\ \hline
Adressa \citep{gulla2017adressa} & 640K    & 20K     \\ \hline
Movielens-25M\footnote{https://grouplens.org/datasets/movielens/25m/}                     & 162K    & 62K     \\ \hline
Yelp \footnote{}                            & 5224    & 7741    \\ \hline
Amazon-Kindle\footnote{}                     & 7650    & 9173    \\ \hline
\end{tabular}
\end{table}

==> tables/general.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}
%\centering
\caption{\textbf{Server model accuracy on MNIST (E=20, K=10) and FEMNIST (E=20, K=10) with full FEDAVG, \name, and LowRank:} test accuracy results of different model compression settings compared to (uncompressed) full FEDAVG on both MNIST and FEMNIST datasets. The notation ``$M_1\times$-$M_2\times$-..." is the same as described in Table \ref{tab:server-fair}. \vspace{6pt}
}\label{tab:general}

\resizebox{\linewidth}{!}{

\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\textbf{Dataset}                               & \textbf{\begin{tabular}[c]{@{}c@{}}Full-FEDAVG\\  Test Acc\end{tabular}}    & \textbf{COMP} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}c@{}}\name\\  Test Acc\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}LowRank\\  Test Acc\end{tabular}}     & \textbf{COMP}     & \textbf{\begin{tabular}[c]{@{}c@{}}\name\\  Test Acc\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}LowRank\\  Test Acc\end{tabular}} \\ \hline
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}MNIST\\  (E=20, K=10)\end{tabular}}}   & \multirow{3}{*}{0.9841} & $4\times$           & 0.9829                                             & \textbf{0.9836} & $2\times$-$4\times$                & 0.9822                        & \textbf{0.9839}  \\ \cline{3-8} 
                                               &                         & $8\times$           & 0.9799                                             & \textbf{0.9829} & $2\times$-$4\times$-$8\times$             & 0.9823                        & \textbf{0.984}   \\ \cline{3-8} 
                                               &                         & $64\times$          & 0.962                                              & \textbf{0.9833} & $2\times$-$4\times$-$8\times$-$16\times$-$32\times$-$64\times$ & 0.9636                        & \textbf{0.9839}  \\ \hline
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}FEMNIST\\  (E=20, K=10)\end{tabular}}} & \multirow{3}{*}{0.7491} & $4\times$           & \textbf{0.7847}                                    & 0.7573          & $2\times$-$4\times$                & \textbf{0.7842}               & 0.7804           \\ \cline{3-8} 
                                               &                         & $8\times$           & \textbf{0.779}                                     & 0.7022          & $2\times$-$4\times$-$8\times$             & \textbf{0.7691}               & 0.7689           \\ \cline{3-8} 
                                               &                         & $64\times$          & \textbf{0.7114}                                    & NA             & $2\times$-$4\times$-$8\times$-$16\times$-$32\times$-$64\times$ & \textbf{0.7409}               & NA               \\ \hline
\end{tabular}
}
\end{table*}

==> tables/goodreads.tex <==
\begin{table}
\caption{Goodreads datasets for federated learning. We propose the following three different sized datasets extracted from Goodreads datasets The mean rating of each datasets is around $3.7$ with a standard deviation around $1$}
\centering
\label{tab:my-table}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Dataset} & \textbf{\#users} & \textbf{\#items} & \textbf{\#interactions} \\ \hline
Goodreads        & 876K             & 2.3M             & 100M                    \\ \hline
Goodreads-S  & 100              & 358K             & 694K                    \\ \hline
Goodreads-L & 1000             & 757K             & 3.3M                    \\ \hline
%goodreads-large  & 10000            & 1.37M            & 15M                     \\ \hline
\end{tabular}
\end{table}
